Shape optimization for contact problems in linear elasticity

This thesis deals with shape optimization for contact mechanics. More specifically, the linear elasticity model is considered under the small deformations hypothesis, and the elastic body is assumed to be in contact (sliding or with Tresca friction) with a rigid foundation. The mathematical formulations studied are two regularized versions of the original variational inequality: the penalty formulation and the augmented Lagrangian formulation. In order to get the shape derivatives associated to those two non-differentiable formulations, we suggest an approach based on directional derivatives. Especially, we derive sufficient conditions for the solution to be shape differentiable. This allows to develop a gradient-based topology optimization algorithm, built on these derivatives and a level-set representation of shapes. The algorithm also benefits from a mesh-cutting technique, which gives an explicit representation of the shape at each iteration, and enables to apply the boundary conditions strongly on the contact zone. The different steps of the method are detailed. Then, to validate the approach, some numerical results on two-dimensional and three-dimensional benchmarks are presented.

==> fonctions_regularisees.tex <==
\chapter{Propriétés des fonctions régularisées}     % numérotée
\label{app:RegFunctions}                            % étiquette pour renvois (à compléter!)


Dans cette annexe, nous donnons les définitions des fonctions régularisées introduites au chapitre \ref{chap:2.2}, ainsi que certaines de leurs propriétés. 

\subsubsection{Terme normal}
Tout d'abord, $\maxxc$ est défini par:
\begin{equation*}
  \maxxc(x) := 
    \left\{
      \begin{array}{lr}
        x- \frac{1}{2c} & \mbox{si} \: x \geq \frac{1}{c}, \\
        c\frac{x^2}{2} & \mbox{si} \: 0 \leq x \leq \frac{1}{c}, \\
        0 & \mbox{sinon.}
      \end{array}
    \right.
\end{equation*}
Ce qui donne pour sa primitive $\psi_c$ (s'annulant en $0$) et sa dérivée $H_c$:
\begin{equation*}
  \psi_c(x) = 
    \left\{
      \begin{array}{lr}
        \frac{x^2}{2}-\frac{1}{2c}x+\frac{1}{6c^2} & \mbox{si} \: x \geq \frac{1}{c}, \\
        \frac{c}{6}x^3 & \mbox{si} \: 0 \leq x \leq \frac{1}{c}, \\
        0 & \mbox{sinon.}
      \end{array}
    \right.
  \hspace{1em}
  H_c(x) = 
    \left\{
      \begin{array}{lr}
       1 & \mbox{si} \: x \geq \frac{1}{c}, \\
        cx & \mbox{si} \: 0 \leq x \leq \frac{1}{c}, \\
        0 & \mbox{sinon.}
      \end{array}
    \right.
\end{equation*}
On peut montrer facilement que ces fonctions vérifient:
%\begin{itemize}[parsep=0.05cm,itemsep=0.05cm,leftmargin=*]
\begin{itemize}[parsep=0.05cm,itemsep=0.05cm]
  \item[(i)] $\maxxc$, $\psi_c$ et $H_c$ sont positives,
  \item[(ii)] pour tout $x \in \mathbb{R}$, $x \maxxc(x) \geq 0$,
  \item[(iii)] $\maxxc$ et $\psi_c$ sont convexes,
  \item[(iv)] pour tout $x \in \mathbb{R}$, $\maxxc(x) \leq \maxx(x) \leq |x|$,
  \item[(v)] $\norml \: \maxxc - \maxx \normr_\infty \leq \frac{1}{8c}$.
\end{itemize}

\subsubsection{Terme tangentiel}
Nous donnons maintenant la définition de la régularisation $\qq_c$ associée à la contrainte tangentielle:
\begin{equation*}
  \qq_c(\alpha,z) := \left\{
      \begin{array}{lr}
        z & \mbox{ si } \: |z| \leq \alpha -\frac{1}{c} ,\\
        \big[ \alpha + P_c(|z|-\alpha) \big] \frac{z}{|z|} & \mbox{ si } \: \alpha -\frac{1}{c} \leq |z| \leq \alpha +\frac{1}{c}, \\
        \alpha \frac{z}{|z|} & \mbox{ si } \: |z| \geq \alpha +\frac{1}{c}. 
        \end{array}
    %   \begin{aligned}
    %     &z & \mbox{ si } \: |z| \leq \alpha -\frac{1}{c}\: ,\\
    %     & \big[ \alpha + P_c(|z|-\alpha) \big] \frac{z}{|z|} & \mbox{ si } \: \alpha -\frac{1}{c} \leq |z| \leq \alpha +\frac{1}{c}\: , \\
    %     &\alpha \frac{z}{|z|} & \mbox{ si } \: |z| \geq \alpha +\frac{1}{c}\: .
    %   \end{aligned}
    \right.
\end{equation*}
Le polynôme $P_c$ est défini par $P_c(t) := -\frac{c}{4}t^2 + \frac{1}{2}t - \frac{1}{4c}$ et il vérifies donc $P_c\left(-\frac{1}{c}\right)=-\frac{1}{c}$,  $P_c'\left(-\frac{1}{c}\right)=1$, $P_c\left(\frac{1}{c}\right)=P_c'\left(\frac{1}{c}\right)=0$, et $-\frac{1}{c}\leq P_c\leq 0$ sur l'intervalle $\left[ -\frac{1}{c}, \frac{1}{c}\right]$.

Afin de pouvoir écrire l'énergie mécanique associée à la formulation pénalisée régularisée, nous avons introduit précédemment $h_c$, la primitive $\frac{1}{\varepsilon}\qq(\varepsilon\mathfrak{F}s,\cdot)$ qui s'annule en $0$. Cette fonction vérifie, pour tout $z\in\mathbb{R}^{d-1}$:
\begin{equation*}
  h_c(z) := \frac{1}{\varepsilon} \left\{
      \begin{array}{lr}
        \frac{1}{2}|z|^2 & \mbox{ si } \: |z| \leq \varepsilon\mathfrak{F}s -\frac{1}{c}\: ,\\
        \varepsilon\mathfrak{F}s |z| + Q_c(|z|-\varepsilon\mathfrak{F}s)- \frac{1}{2} (\varepsilon\mathfrak{F}s)^2  & \mbox{ si } \: \varepsilon\mathfrak{F}s -\frac{1}{c} \leq |z| \leq \varepsilon\mathfrak{F}s +\frac{1}{c} ,\\
        \varepsilon\mathfrak{F}s |z| - \frac{1}{2} (\varepsilon\mathfrak{F}s)^2 - \frac{1}{6c} & \mbox{ si } \:  |z| \geq \varepsilon\mathfrak{F}s +\frac{1}{c}\: ,
      \end{array}
    \right.
\end{equation*}
où $Q_c$ est la primitive de $P_c$ qui s'annule en $0$.

Par souci de lisibilité, nous introduisons les trois sous-ensembles de  $\mathbb{R}_+^*\times\mathbb{R}^{d-1}$ suivants: $\pazocal{J}^{c,-}:=\{ (\alpha,z) \mbox{ s.t. } |z| \leq \alpha -\frac{1}{c} \}$, $\pazocal{J}^{c,0}:=\{(\alpha,z) \mbox{ s.t. } \alpha -\frac{1}{c} \leq |z| \leq \alpha +\frac{1}{c} \}$ et $\pazocal{J}^{c,+}:=\{(\alpha,z) \mbox{ s.t. } |z| \geq \alpha +\frac{1}{c} \}$.

On peut exprimer les dérivées partielles de $\qq_c$ par rapport à $\alpha$ et $z$, notées respectivement $\partial_\alpha\qq_c : (\frac{1}{c},+\infty)\times\mathbb{R}^{d-1} \to \mathcal{L}(\mathbb{R};\mathbb{R}^{d-1})$ et $\partial_z \qq_c :(\frac{1}{c},+\infty) \times\mathbb{R}^{d-1} \to \mathcal{L}(\mathbb{R}^{d-1})$, de la manière suivante:
\begin{equation*}
  \partial_\alpha \qq_c(\alpha,z) = \left\{
      \begin{array}{lr}
        0 & \mbox{ in } \pazocal{J}^{c,-} ,\\
        \big[ 1 - P_c'(|z|-\alpha) \big] \frac{z}{|z|} & \mbox{ in } \pazocal{J}^{c,0}\: , \\
        \frac{z}{|z|} & \mbox{ in } \pazocal{J}^{c,+} ,
      \end{array}
    \right.
\end{equation*}
\begin{equation*}
  %\partial_z \qq_c(\alpha,z) = 
  \partial_z \qq_c(\alpha,z) = \left\{
      \begin{array}{lr}
           I_{d-1} & \mbox{in } \pazocal{J}^{c,-}, \\
           \frac{1}{|z|^2} P_c'(|z| - \alpha)z \otimes  z & \: \\
           \qquad + \frac{1}{|z|} \big[ \alpha + P_c(|z| - \alpha) \big] \big(I_{d-1}  -  \frac{1}{|z|^2} z \otimes  z\big)& \mbox{in } \pazocal{J}^{c,0}\:, \\
           \frac{\alpha}{|z|}\big(I_{d-1}  -  \frac{1}{|z|^2} z \otimes  z\big) & \mbox{in } \pazocal{J}^{c,+},
      \end{array}
    \right.
\end{equation*}
où $I_{d-1}$ correspond à la matrice identité de taille $d-1$.

Nous énonçons maintenant quelques propriétés utiles de ces fonctions:
\begin{itemize}[parsep=0.05cm,itemsep=0.05cm]
    \item[(i)] $h_c$ est convexe,
    \item[(ii)] pour tous $\alpha\in\mathbb{R}_+^*$, $z\in\mathbb{R}^{d-1}$, $\qq_c(\alpha,z)z \geq 0$,
    \item[(iii)] pour tous $\alpha\in\mathbb{R}_+^*$, $z\in\mathbb{R}^{d-1}$, $|\qq_c(\alpha,z)| \leq |\qq(\alpha,z)|\leq\alpha$ et $|z|$,
    \item[(iv)] pour tous $\alpha\in\mathbb{R}_+^*$, $z,z'\in\mathbb{R}^{d-1}$, $(\qq(\alpha,z)-\qq(\alpha,z'))(z-z')\geq 0$,
    \item[(v)] pour tout $\alpha\in\mathbb{R}_+^*$, $\norml \qq_c(\alpha,\cdot)- \qq(\alpha,\cdot)\normr_\infty\leq \frac{2}{c}$,
    \item[(vi)] $\partial_\alpha \qq_c$ et $\partial_z \qq_c$ sont continues sur $(\frac{1}{c},+\infty)\times\mathbb{R}^{d-1}$,
    \item[(vii)] $\partial_\alpha \qq_c$ et $\partial_z \qq_c$ sont uniformément bornées,
    \item[(viii)] $\qq_c$ est Lispschitz sur $(\frac{1}{c},+\infty)\times\mathbb{R}^{d-1}$,
    \item[(ix)] $\partial_\alpha\qq_c $ est Lispschitz sur $(\frac{1}{c},+\infty)\times\mathbb{R}^{d-1}$,
    \item[(x)] il existe $K>0$ tel que, pour tous $\alpha, \alpha'\in(\frac{1}{c},+\infty)$, $z, z'\in\mathbb{R}^{d-1}$,
    \vspace{-0.5em}
    \begin{equation*}
        |\partial_z \qq_c(\alpha,z)-\partial_z \qq_c(\alpha',z')|\leq Kc\left( \left| (\alpha,z)-(\alpha',z')\right| + \left| (\alpha,z)-(\alpha',z')\right|^2 \right).
    \end{equation*}
\end{itemize}

\begin{rmrk}
    Puisque $\qq_c$ a des dérivées partielles continues, elle est différentiable, et sa dérivée directionnelle en $(\alpha,z)$ dans n'importe quelle direction $(\beta,h)\in\mathbb{R}\times\mathbb{R}^{d-1}$ s'écrit:
    \begin{equation*}
        \qq_c'\left((\alpha,z);(\beta,h)\right) = \partial_\alpha\qq_c(\alpha,z)\beta+\partial_z\qq_c(\alpha,z)h\:.
    \end{equation*}
\end{rmrk}

\begin{proof}
    (\textit{Propriétés de $\qq_c$ et de ses dérivées partielles}) Les cinq premières propriétés son immédiates. Nous nous concentrons sur les quatre suivantes.
    
    (vi): Compte tenu des expressions des dérivées partielles, on peut déduire que, pour tout $(\alpha,z)\in \mathbb{R}_+^*\times\mathbb{R}^{d-1}$, la forme bilinéaire associée à $\partial_z \qq_c(\alpha,z)$ est positive sur $\mathbb{R}^{d-1} \times \mathbb{R}^{d-1}$. Il est clair que si $\pazocal{J}^{c,-} = \emptyset$, ce qui est le cas quand $\alpha < \frac{1}{c}$, ces dérivées ne sont pas continues par rapport à $z$ (problème en $z=0$). Ainsi, on a que  $\partial_\alpha \qq_c$ et $\partial_z \qq_c$ sont toutes les deux continues sur $(\frac{1}{c},+\infty)\times\mathbb{R}^{d-1}$.
    
    (vii): pour tout $(\alpha,z) \in \mathbb{R}_+^*\times\mathbb{R}^{d-1}$, puisque $\norml z\otimes z \normr \leq |z|^2$, on obtient:
    \begin{equation*}
        | \partial_\alpha\qq_c(\alpha,z) | \leq 1 \: , \hspace{3em} \norml \partial_z \qq_c(\alpha,z) \normr \leq 3 \: .
    \end{equation*}
   
    (viii): Soient $(\alpha,z)$ et $(\alpha',z') \in \mathbb{R}_+^*\times\mathbb{R}^{d-1}$, la propriété (vii) permet d'obtenir la majoration suivante:
    \begin{equation*}
        \begin{aligned}
        \left| \qq_c(\alpha',z') - \qq_c(\alpha,z) \right| &\leq \:\left| \qq_c(\alpha',z') - \qq_c(\alpha,z') \right| + \left| \qq_c(\alpha,z') - \qq_c(\alpha,z) \right| \: ,\\
        \: & \leq \: \sup_{\alpha} | \partial_\alpha\qq_c(\alpha,z) | \cdot |\alpha' - \alpha| + \sup_{z} \norml \partial_z \qq_c(\alpha,z) \normr \cdot |z'-z| \: ,\\
        \: & \leq \: 3 | (\alpha',z') - (\alpha,z) | \: .
    \end{aligned}
    \end{equation*}
    
    (ix) et (x): Pour démontrer ces deux dernières propriétés, il suffit de procéder par disjonction des cas, puis de développer les calculs. Nous choisissons de ne pas détailler ces preuves, car elles sont assez fastidieuses, et ne présentent pas un grand intérêt.
    
\end{proof}



